The Molecular Cloud Lifecycle I: Constraining H2 formation and dissociation rates with observations

Molecular clouds (MCs) are the birthplaces of new stars in galaxies. A key component of MCs are photodissociation regions (PDRs), where far-ultraviolet radiation plays a crucial role in determining the gas's physical and chemical state. Traditional PDR models assume chemical steady state (CSS), where the rates of H$_2$ formation and photodissociation are balanced. However, real MCs are dynamic and can be out of CSS. In this study, we demonstrate that combining H$_2$ emission lines observed in the far-ultraviolet or infrared with column density observations can be used to derive the rates of H$_2$ formation and photodissociation. We derive analytical formulae that relate these rates to observable quantities, which we validate using synthetic H$_2$ line emission maps derived from the SILCC-Zoom hydrodynamical simulation. Our method estimates integrated H$_2$ formation and dissociation rates with an accuracy $\approx 30$ % (on top of uncertainties in observed H$_2$ emission maps and column densities). Our simulations, valid for column densities $N \leq 2 \times 10^{22}$ cm$^{-2}$, cover a wide dynamic range in H$_2$ formation and photodissociation rates, showing significant deviations from CSS, with 74 % of the MC's mass deviating from CSS by a factor greater than 2. Our analytical formulae can effectively distinguish between regions in and out of CSS. When applied to actual H$_2$ line observations, our method can assess the chemical state of MCs, providing insights into their evolutionary stages and lifetimes. A NASA Small Explorer mission concept, Eos, will be proposed in 2025 and is specifically designed to conduct the types of observations outlined in this study.

==> applications_to_W43.tex <==
\subsection{Application to observations}
\label{sub: diss W43}
As an example, let us consider the W43 star-forming region.
W43 is an exceptionally active star-forming region, housing numerous MCs and atomic gas, located at the intersection of the Galactic bar with the first spiral arm, towards the Galactic center  ($l = 29.2-31.5^{\circ}$, $|b| \leq 1^{\circ}$; $d=5.5\pm0.5$ kpc) \citep{Motte2003, NguyenLuong2011, Carlhoff2013}.
The HI column density observed towards W43 is abnormally large, with $N({\rm HI})$ reaching values as high as $\approx 2 \times 10^{22}$ cm$^{-2}$ \citep{Bihr2015}. This is in tension with theoretical models of equilibrium  HI-H$_2$ transition, which predict an order of magnitude smaller HI columns \citep[][]{Krumholz2009, Sternberg2014}.

\citet{Bialy2017b} discuss two possibilities for solving this discrepancy. In the first scenario, W43 is modeled as an ensemble of HI-to-H$_2$ transition layers (or equivalently photodissociation regions; PDRs). Each PDR is in a chemical equilibrium and produces a moderate HI column of order $N({\rm HI}) \approx 10^{21}$ cm$^{-3}$ \citep[see Fig 2 in][]{Bialy2017b}. The superposition of several PDRs along the LOS gives rise to the large HI column densities observed.
In the second scenario, the large observed HI columns are seen as a transient phenomenon where the HI is in the process of converting to H$_2$, and the system hasn't yet had time to reach a chemical equilibrium (i.e., this is in line with the dynamic scenario discussed in \citealt{Motte2014}).

The question of whether the HI is produced in several chemically steady HI layers or in a dynamically forming cloud (i.e., scenarios I vs II), has implications for the cloud's lifetime. In the first scenario, the cloud is relatively old, with $t_{\rm cloud} \gg t_{\rm chem}$, and has achieved a chemical equilibrium. In the second scenario, the cloud is young, with $t_{\rm cloud} \ll t_{\rm chem}$, and is still in its assembly process.

The emission power in H$_2$ lines may be used to determine between these two scenarios (see also \S 4.2 in \citealt{Bialy2017b}).
According to Eq.~(\ref{eq: JF_to_JD IR}), if the system is in a chemical equilibrium ($J_F=J_D$), then the total power in H$_2$ IR lines is
\begin{equation}
    I_{5} = 1.4 N_{21}^{1+\alpha} f_{\rm H} \left( \frac{1-\mathrm{e}^{-\tau_{\rm tot}}}{\tau_{\rm tot}} \right) \ .
\end{equation}
For W43,  $N_{21} \approx 20$ and $f_{\rm H} \approx 0.3$ (see Fig.~17 in \citealt{Bihr2015}), and we get that for the equilibrium scenario to hold the total line emission in the IR should be 
$I_{\rm tot, IR} \approx 2.7 \times 10^{7} \ {\rm photons \ cm^{-2} \ s^{-1} \ sr^{-1}}$, where we assumed $\tau_{\rm tot}\approx 0.9$, corresponding to $\sigma= 4.5 \times 10^{-23}$ cm$^2$ appropriate to the wavelength range $\lambda=2-3$ $\mu$m \citep{Draine2011}. 


If, on the other hand, we observe line emission power that is significantly lower than the value above, this would provide evidence in favor of the second scenario, where the HI-H$_2$ is not in a chemical equilibrium in W43, and the molecular gas is in its active formation phase, i.e., scenario II.

